Contemporary COBOL: Developers' Perspectives on Defects and Defect Location

Mainframe systems are facing a critical shortage of developer workforce as the current generation of COBOL developers retires. Furthermore, due to the limited availability of public COBOL resources, entry-level developers, who assume the mantle of legacy COBOL systems maintainers, face significant difficulties during routine maintenance tasks, such as code comprehension and defect location. While we made substantial advances in the field of software maintenance for modern programming languages yearly, mainframe maintenance has received limited attention. With this study, we aim to direct the attention of researchers and practitioners towards investigating and addressing challenges associated with mainframe development. Specifically, we explore the scope of defects affecting COBOL systems and defect location strategies commonly followed by COBOL developers and compare them with the modern programming language counterparts. To this end, we surveyed 30 COBOL and 74 modern Programming Language (PL) developers to understand the differences in defects and defect location strategies employed by the two groups. Our preliminary results show that: (1) major defect categories affecting the COBOL ecosystem are different than defects encountered in modern PL software projects; (2) the most challenging defect types in COBOL are also the ones that occur most frequently; and (3) COBOL and modern PL developers follow similar strategies to locate defective code.

==> methodology.tex <==
\section{Research methodology}
To capture developers' perspective on software defects and defect location strategies, we leveraged prior research to devise taxonomies characterizing each of the two dimensions~\cite{catolino2019,odc,morrison2018,wang2013}. To ensure that the taxonomies correspond with developers' experience and practices, we consulted one COBOL and one non-COBOL developer, and altered the taxonomies accordingly. In this section, we describe the process of building and refining taxonomies used in the study.


\subsection{Software defects taxonomy}
Previous research have identified taxonomies characterizing software defects at different levels of granularity and with various properties ~\cite{odc,catolino2019,freimut2005,grady1992}. 
In this study, we leverage bug classification schema proposed by Catolino et al.~\cite{catolino2019}. This schema comprises of 9 defect categories, namely Configuration, Database, GUI, Network, Performance, Permission/Deprecation, Program Anomaly, Security and Test Code, hence it provides concise, yet comprehensive selection of defect types. However, we identified two major drawbacks of applying this taxonomy in our study. Firstly, as pointed out by Catolino et al., Program Anomaly is a broad category and pertain to the majority of software bugs. Moreover, the same concern was raised by participants of the pilot study. Hence, based on defect types indicated during the pilot study, we decided to expand Program Anomaly into 3 categories. Input data refers to issues caused by unexpected or malformed input data, which often occurs in COBOL ecosystem. Concurrency-related defects involves bugs related to e.g., incorrect access to shared resources or deadlocks, while Logic/Flow defects pertain to programming errors, e.g., incorrect use of data structures. Additionally, as indicated by the participants of the pilot study, we also introduced a new category related to defect occurring when system operates at the limit of the resources, Workload/Stress. In total, in the study we use 11 defect categories as shown in Tab.~\ref{tab:defects-taxonomy}.

To capture properties of software defects, we leverage Orthogonal Defect Classification (ODC)~\cite{odc}. ODC describes defect properties at two moments in time (opening section), when defect is reported and when it is closed (closing section). 
Although, this taxonomy captures fine-grained details of defects, it is not applicable in a context of a survey since it requires participants to be familiar with its extensive terminology. Therefore, we opted for a hybrid approach in which we leverage defect categories based on the work of Catolino et al.~\cite{catolino2019}, which to some extent covers opening section properties, and additionally, we also use three of the closing section dimensions, Age, Source and Qualifier. In particular, Age refers to the time when defect was introduced into the code base, Source indicates which part of code was affected, while Qualifier identifies the cause of the defect. Comparing to the options specified in ODC for each of these dimensions, we decided to introduce two changes. First, we introduce Corrupted Data as a Qualifier to capture one of the frequent cause of defects in COBOL projects. Secondly, we merge Outsourced and Ported from the Source dimension into one category, Outsourced. The modification was dictated by observing participant of the pilot study who had difficulties in differentiatign between the two options.
Finally, following Morrison et al.~\cite{morrison2018}, we introduced a dimension to determine an entity that reported a defect, Reporter. The final version of defect location taxonomy is presented in Tab.~\ref{tab:defects-taxonomy} and includes categories of defects and their properties.
 

\begin{table}[ht]
\scriptsize
\caption{Software defects taxonomy based on \cite{catolino2019} and \cite{odc}.}
\label{tab:defects-taxonomy}
\begin{tabular}{l|ll}
\toprule
\textbf{Defect categories} & \multicolumn{2}{l}{\textbf{Defect properties}} \\ \midrule
Concurrency & \multirow{3}{*}{Reporter} & Developer \\
Configuration &  & Quality Assurance Personnel/ Tester \\
Database &  & End user \\ \cline{2-3}
GUI & \multirow{4}{*}{Cause} & Not coded to specification \\
Input Data &  & Missing or incomplete specification \\
Logic/Flow &  & Corrupted data \\ 
Network &  & Extraneous \\ \cline{2-3}
Performance & \multirow{3}{*}{Source} & Developed in-house \\
Permission/Deprecation &  & External library/API \\
Security &  & Outsourced \\ \cline{2-3}
Test Code & \multirow{4}{*}{Age} & New feature \\
Workload/Stress &  & Legacy code \\
 &  & Re-factored \\
 &  & Changed to fix a defect \\ \bottomrule
\end{tabular}
\end{table}
\subsection{Defect location taxonomy}


To study the process of defect location from a perspective of a software developer, researchers conducted exploratory studies to observe developers' actions when working on maintenance tasks \cite{ko2006,sillito2008, wang2013,kevic2017}. The summary of identified developer activities is presented in Table~\ref{tab:activities}. We note that across all of the examined studies exist a shared set of activities that reflect the process of locating a feature in code. More specifically, in all of the studies, the authors observed developers looking for a code entity representing a starting point (Seek, Search, Finding focus point, Searching for a specific string), followed by exploring related program elements (Relate, Expand, Expanding focus points)~\cite{ko2006,wang2013, sillito2008}. Additionally, 2 out of 4 studies identified documenting relevant code entities by developers \cite{ko2006,wang2013}. Overall, across various research we note a set of common high-level activities performed by developers when locating a feature.


\begin{table}[t]
\centering
\scriptsize
\caption{Stages of defect (or feature) location process identified in the previous studies.}
\label{tab:activities}
\begin{tabular}{p{0.5cm}p{0.5cm}p{1.3cm}p{1.5cm}}
\toprule
\multicolumn{1}{l}{Ko et al.~\cite{ko2006}} & \multicolumn{1}{l}{Wang et al. \cite{wang2013}} & \multicolumn{1}{l}{Sillito et al. \cite{sillito2008}}        & \multicolumn{1}{l}{Kevic et al. \cite{kevic2017}}     \\ \midrule
Seek                   & Search                   & Finding focus point                & Understanding of source code  \\
Relate                 & Expand                   & Expanding focus point              & Changes to source code         \\
Collect                & Validate                 & Understanding a subgraph           & Change task examination       \\
                       & Document                 & Questions over a graph of subgraph & Searching for specific string \\ \bottomrule
\end{tabular}
\end{table}

%Researchers observed that feature location is a highly iterative process with developers interleaving activities~\cite{wang2013,ko2006}.



In this study, we decided to leverage hierarchical feature location model proposed by Wang et al.~\cite{wang2013}. 
We deem this model serves as a good starting point as it (1) captures feature location process at different levels of granularity; (3) it is based on three exploratory studies with large number of developers; and (3) shares common set of activities with previous studies.
To describe feature location process, the authors used three levels of granularity: phases, patterns and actions. Each phase represent a high-level stage in a feature location process, namely Search for entrance points, Expanding the search, Validating and Documenting. Patterns define common strategies developers follows at different phases related to e.g., execution or textual search, while actions correspond to fine-grained physical or mental activities undertaken by developers. 
Across all the phases, the authors identified 11 physical actions and 6 mental actions. The physical actions included e.g., reading code, or exploring source code files, while mental actions covered e.g., conceiving an execution scenario or identifying and refining keywords.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/locations/paper_drawings.pdf}
    \caption{Defect location model.}
    \label{fig:defect-location-model}
\end{figure*}

Although, this hierarchical model provides a comprehensive representation of behavioral patterns used for locating relevant code entities, we decided to alter some of it components for the purpose of this study. The goal of these changes was (1) to create more concise representation of the model; and (2) to capture additional activities as indicated by the participants of the pilot study.
Figure~\ref{fig:defect-location-model} presents the overview of the model with phases containing available patterns, while actions and strategies are listed below each phase. We mark introduced modifications with red color.
In general, we reuse all of the phases defined in the original model, however, we extend available patterns. In particular, we included the IR-based pattern in the Expanding the search phase for the symmetry with the Search phase. Researchers noted that developers tend to lost track of the relevant program elements due to the large number of examined files and interruptions~\cite{ko2006,wang2013,sillito2008,latoza2006}. To provided more context for the Documentation phase and investigate if and how developers collect the information about relevant code components, we curated a list of common practices for documenting code based on prior work~\cite{ko2006, wang2013}.

We modified the original list of physical actions in a following manner. We decided to merge {\em Breakpoints operations}, {\em Step program} and {\em Run program} into one succinct action, {\em Observing runtime}. As noted by Kr\"{u}ger et al.~\cite{kruger2018}, location of a specific feature can be discovered by examining the release log and pull requests, thus to reflect that we added new physical action, {\em Examine VCS}. 


%For instance, in the case for IR-based search patterns, we distinguished two types of a query: natural language description and name of a source code artifact~\cite{}, while exploration-based patterns was divided into navigating static dependencies and navigating through files, as suggested in \cite{ko2006}. 


% "Overall, developers spent about half of their time searching for entrance points, forth of their time extending the relevant program elements, sixth of their time validating the relevance of program elements, and twelfth of their time documenting their analysis results." wang2013
